Deception through Half-Truths

Deception is a fundamental issue across a diverse array of settings, from cybersecurity, where decoys (e.g., honeypots) are an important tool, to politics that can feature politically motivated "leaks" and fake news about candidates.Typical considerations of deception view it as providing false information.However, just as important but less frequently studied is a more tacit form where information is strategically hidden or leaked.We consider the problem of how much an adversary can affect a principal's decision by "half-truths", that is, by masking or hiding bits of information, when the principal is oblivious to the presence of the adversary. The principal's problem can be modeled as one of predicting future states of variables in a dynamic Bayes network, and we show that, while theoretically the principal's decisions can be made arbitrarily bad, the optimal attack is NP-hard to approximate, even under strong assumptions favoring the attacker. However, we also describe an important special case where the dependency of future states on past states is additive, in which we can efficiently compute an approximately optimal attack. Moreover, in networks with a linear transition function we can solve the problem optimally in polynomial time.

==> flipping.tex <==
\subsection{Flipping}
The results presented throughout the paper pertaining to the hiding outcomes, are easily extended to an attacker who is aloud to flip outcomes rather than hiding them.

First, there are a few propositions that follow immediately from their half-truth counterparts.
Proposition \ref{prop:arb} shows that a myopic observer can be made to incur arbitrarily high loss by simply hiding some fraction of the nodes in $\bold{X}^0$. This result also holds for an attacker who can only flip outcomes.

Additionally, the hardness results discussed in Propositions \ref{P=NP} and \ref{RP=NP} show that no polynomial approximation of the optimal solution can be computed in polynomial time, using either a deterministic or randomized algorithm, unless $P = NP$ or $RP = NP$, respectively.
We obtain equivalent results for the case when the adversary can hide nodes.

\begin{proposition}
Suppose that in the DBNM problem the adversary is finding a mask which corresponds to outcomes that will be changed rather than hidden. The hardness results from propositions \ref{P=NP} and \ref{RP=NP} hold true for this setting as well.
\end{proposition}
\begin{proof}
This result follows immediately from proofs of Propositions \ref{P=NP} and \ref{RP=NP}.
\end{proof}


In addition to this hardness result, we also have an equivalent hardness result for the additive case discussed in Section \ref{sec:add}. That is, in an almost identical statement to Proposition 
\ref{prop:add_hard}:

\begin{proposition}
No PTAS exists for the flipping version of of PDBNM, (even for monotone transition functions, when nodes have at most 2 parents).
\end{proposition}

\begin{proof}
Follows immediately from the proof of Proposition 
\end{proof}



First we will discuss the case when the adversary is able to flip the outcomes of up to $k$ nodes. For any mask $\eta$, let $\Delta(X_j^0)$ represent the change in the attacker's utility when $X_j^0$ is added to $\eta$.
\begin{algorithm} 
\caption{Approximation algorithm}
\begin{algorithmic}[1]\label{alg:flip_appro}
\State bestMask := $\emptyset$
\For{\textbf{each} $X_i^1 \in \bold{X}^1$}

    \State $S_0 = \{ X_j^0 \in \Pa(X_i^1): \phi(X_j^0) = 0\}$
    \State $S_1 = \{ X_j^0 \in \Pa(X_i^1): \phi(X_j^0) = 1\}$
    
    \State $\eta_0 := \emptyset$
    \State $\eta_1 := \emptyset$
    \State \textbf{let} $z_i^{\eta}$ be the $z_i$ induced by $\eta$
    
    \While{$S_0 \setminus \eta_0 \neq \emptyset$ and $|\eta_0| \leq k$}
        
        \State add $s \in S_0$, with maximal $\Delta(s)$, to $\eta_0$
        \If{$V(\eta_0) > V(\text{bestMask})$}
            \State bestMask $:= \eta_0$
        \EndIf
    \EndWhile
    \While{$|\eta_0| < k$}
        \State add $X_j^0 \in \bold{X}$, with maximal $\Delta(X_j^0)$ to $\eta_0$
        \If{$V(\eta_0) > V(\text{bestMask})$}
            \State bestMask $:= \eta_0$
        \EndIf
    \EndWhile
    
    \While{$S_1 \setminus \eta_1 \neq \emptyset$ and $|\eta_1| \leq k$}
        
        \State add $s \in S_1$, with maximal $\Delta(s)$, to $\eta_1$
        \If{$V(\eta_1) > V(\text{bestMask})$}
            \State bestMask $:= \eta_1$
        \EndIf
    \EndWhile
    \While{$|\eta_1| < k$}
        \State add $X_j^0 \in \bold{X}$, with maximal $\Delta(X_j^0)$ to $\eta_1$
        \If{$V(\eta_1) > V(\text{bestMask})$}
            \State bestMask $:= \eta_1$
        \EndIf
    \EndWhile

\EndFor
\Return bestMask
\EndProcedure

\end{algorithmic}
\end{algorithm}

In words, the above algorithm looks at each parent set of nodes $\Pa(X_i^1)\in \bold{X}^0$. Each set is then partitioned based the outcomes assigned by $\phi$. On each of the two partitions we then perform a local search for the most optimal mask by greedily adding the element from each partition that provides the largest increase to the attacker's total utility. If the budget $k$ is not fully spent, we continue greedily adding nodes from $\bold{X}^0$ until the budget is expended. As each node is added to the mask, we keep track of which mask provided the maximum utility and then return that mask at the end of the algorithm.

\begin{proposition}\label{prop:flip_appro}
Algorithm \ref{alg:flip_appro} achieves an $n-$approximation of the optimal solution when $\eta$ is the set of nodes to have their outcomes flipped.
\end{proposition}

\begin{proof}
    For a given outcome map, $\phi$, let $z_i^* = \sum_{X_j^0\in \Pa(X_i^1)}\phi(X_j^0)$ and let $X_a^1\in \bold{X}^1$ be the node with the largest value of 
    
    $$\max\{H\big(\mathbb{P}(X_i^1|z_i^*), \mathbb{P}(X_i^1| r)\big): |r - z_i^*| \leq k\}$$
    For $X_a^1$, denote the $r$ yielding the largest value as $r_a$.
    WLoG assume that $r_a > z_a^*$. Let $d = |r_a - z_a^*|$, then in order for the attacker to have $X_a^1$ contribute $H\big(\mathbb{P}(X_i^1|z_i^*), \mathbb{P}(X_i^1| r)\big)$ to the total utility, the attacker would have to expend $d$ of the budget. As per definition of $r_a$, $d \leq k$. Therefore, when the algorithm is constructing a mask over $\Pa(X_i^1)$, it will pick up $d$ elements from $S_0$, flipping them to $1$'s.
    Therefore, at some iteration, a mask is constructed with at least value $H\big(\mathbb{P}(X_a^1|z_a^*), \mathbb{P}(X_a^1| r_a)\big)$. Since the mask with the maximum utility is returned, the value of the mask produced by this algorithm is at least $H\big(\mathbb{P}(X_a^1|z_a^*), \mathbb{P}(X_a^1| r_a)\big)$.
    Further, since the attacker's total utility is given by 
    
    $$ \sum_{i=1}^nH\big(\mathbb{P}(X_i^1|z_i^*), \mathbb{P}(X_i^1| z_i^{\eta})\big)$$
    $$ \leq n H\big(\mathbb{P}(X_a^1|z_a^*), \mathbb{P}(X_a^1| r_a)\big)$$
    
    Therefore, the mask produced by this algorithm obtains at least $\frac{1}{n}$ of the optimal utility. 
    
\end{proof}




\begin{proposition}

If each transition function is given by a linear function 
$$\mathbb{P}(X_i^1 = 1| \phi(\Pa(X_i^1)) = \sum_{X_j^0\in \Pa(X_i^1)}\phi(X_j^0)a_{ij},$$
then the optimal mask $\eta$ can be computed in polynomial time.
\end{proposition}


\begin{proof}
Let $\phi$ be the map given by nature and let $\psi_{\eta}$ be the map defined by $\eta$, that is, $\phi$ and $\psi_{\eta}$ agree on the outcomes of all $X_j^0$, except those in $\eta$. More specifically, if $X_j^0\notin\eta$ then $\psi_{\eta}(X_j^0) = \phi(X_j^0)$ and if $X_j^0 \in \eta$ then $\psi_{\eta}(X_j^0) = 1 - \phi(X_i^0)$.
For $X_i^1 \in \bold{X}^1$, let $Q_i = \sum_{x_j^0\in \Pa(X_i^1)}a_{ij}\phi(X_j^0)$.

Then for any specific $X_i^1 \in \bold{X}^1$ suppose that one of its children $X_r^0$, with $\phi(X_j^0) = 1$ is added to $\eta$, then the change in utility can be expressed as,

$$ 
\sum_{X_j^0 \in \Pa(X_i^1)}\psi_{(\eta\cup \{X_r^0\} )}(X_j^0)a_{i j} + Q_i $$
$$- 2  \sum_{X_j^0 \in \Pa(X_i^1)}\psi_{\eta \cup \{X_r^0\}}(X_j^0)a_{i j} Q_i$$
$$ -\bigg(\sum_{X_j^0 \in \Pa(X_i^1)}\psi_{\eta}(X_j^0)a_{i j} + Q_i - 2  \sum_{X_j^0 \in \Pa(X_i^1)}\psi_{\eta}(X_j^0)a_{i j} Q_i\bigg)
$$

$$ =  
\big(\sum_{X_j^0 \in \Pa(X_i^1)}\psi_{(\eta\cup \{X_r^0\} )}(X_j^0)a_{i j}\big)(1 -  2Q_i) + Q_i-
$$
$$\bigg( \big(\sum_{X_j^0 \in \Pa(X_i^1)}\psi_{\eta}(X_j^0)a_{i j}\big) ( 1 -  2Q_i) + Q_i \bigg)
$$

$$ = \psi_{(\eta \cup \{X_r^0\})}(X_r^0)a_{ir}(1-2Q_i) - \psi_{\eta}(X_r^0)a_{ir}(1-2Q_i)
$$

$$ = a_{ir}(1-2Q_i)
$$

Thus for any $X_i^1 \in \bold{X}^1$ if we hide $X_r^0$ when $\phi(X_r^0) = 0$, then the change in utility to $X_i^1$'s contribution to the total utility is $a_{ir}(1-2Q_i)$, and similarly when $\phi(X_r^0) = 1$, the change is $-a_{ir}(1-2Q_i)$. Note that this change in utility is independent of the current mask $\psi_{\eta}$ and that the total utility is simply the sum of the utility on each $X_i^1$. Thus, when hiding any $X_r^0$ the change in the attacker's total utility increases linearly by a value that depends only on $X_r^0$ and not on the current mask $\eta$. Therefore the attackers utility can be written as 

$$ \sum_{i = 1}^n Q_i + \sum_{r \in \mathbb{I}(\Pa(X_i^1)}y_r(-1)^{\phi(X_r^0)} a_{ir}(1-2Q_i)$$

where $\mathbb{I}(\Pa(X_i^1)$ is the index set of the parents of $X_i^1$, and if $X_r^0 \in \eta$ then $y_r = 1$ and if $X^0_r \notin \eta$ then $y_r = 0$. Assigning values to each $y_r$ such that $\sum_{r = 1}^n y_r \leq k$ can be done in polynomial time by simply selecting the $y_r$'s with the highest associated coefficients.



\end{proof}

==> ilp.tex <==
\subsection{ILP}
\textcolor{blue}{I assume this section can be removed since the ILP is also producing a $n-$approximation and doesn't seem likely to do better. It doesn't seem like the formulation has merit if it cannot improve on results we already have}

In the case when the adversary can flip up to $k$ outcomes, we can formulate the problem as an integer linear program. 
For each each $X_i^1\bold{X}^1$ and a given outcome $\phi$, there are $|\Pa(X_i^1) + 1|$ possible contributions that $X_i^1$ could make to the attackers total utility. Namely, 

$$H\big(\mathbb{P}(X_i^1 = 1| z_i^*), \mathbb{P}(X_i^1=1|a_i)\big) \text{ for } 0 \leq a_i\leq |\Pa(X_i^1)|$$

The goal of the adversary is to choose which $j_i$'s the observer is shown, subject to the constraints that each only one $j_i$ can be selected for each $i$, the $j_i$ that is selected must the the sum of the parents of $X_i$ after the bits are flipped, and that the number of bits flipped cannot be greater than $k$. Thus we can use a variables $x_i$ to represent which outcomes the attacker changes, and $y_{ij}$ to indicate which utility is selected on $X_i$, i.e. which $H\big(\mathbb{P}(X_i^1 = 1| z_i^*), \mathbb{P}(X_i^1=1|j_i)\big)$ is selected. Thus we can formulate this optimization as the following integer linear program.

$$ \text{maximize } \sum_{i=1}^n \sum_{j \in I(\Pa(X_i^1))} y_{ij} H\big(\mathbb{P}(X_i^1 = 1| z_i^*), \mathbb{P}(X_i^1=1|a_i)\big) $$

$$\text{s.t. } \sum_{j \in I(\Pa(X_i^1))}x_j(1 - \phi(X_j^0)) + (1-x_j)(\phi(X_j^0))$$
$$ = \sum_{j\in I(\Pa(X_i^1))}y_{ij}a_i \quad \forall~i$$
$$ \sum_{i = 1}^n x_i \leq k $$
$$ \sum_{j \in I(\Pa(X_i^1))}y_{ij} = 1 \quad \forall~i$$

$$ y_{ij}, x_i \in \{0, 1\} \quad \forall~i, j$$

==> newlimit.tex <==
%\section{Half-Truth is as Good as a Lie}

%In this section we investigate the maximum strength of an attack with respect to both a myopic and rational observer.
Our first result demonstrates that in a fundamental sense, in our model, partially hiding the true current state can lead to arbitrary distortion of belief by a myopic observer.

Recall that the adversary's aim is to maximize statistical distance $D$ between the true posterior distribution over $\bold{X}^1$, and the posterior induced by masking a subset of variables in stage 0, $\bold{X}^1_\eta$.
We now show that for most reasonable measures of statistical distance, we can construct cases in which the adversary can make it arbitrarily large (within limits of the measure itself)---that is, the adversary can induce essentially arbitrary distortion in belief solely by masking some of the observations.

%First, consider the case of optimal adversarial play against a myopic observer, that is, an observer who uses only their prior belief and transition probabilities to make predictions about the next time step.

%Consider an attacker whose objective is to maximize some statistical distance, $D$, between the observer's prediction without obstruction, $\bold{X}^1$, and the observer's prediction when $\eta$ is hidden, $\bold{X}_{\eta}^1$. We will show that if $D$ is positive symmetric, Definition \ref{def:possem}, then there exist networks on which the observer can do arbitrarily well. 




\begin{theorem}%\label{prop:arb}
Suppose the attacker's objective is to maximize some statistical distance $D$ which is bounded from below.
Then there exists a sequence of dynamic Bayes networks, $\bold{X}^0 \rightarrow\bold{X}^1$, with respect to $n$, on which an attacker can do arbitrarily well. More specifically, let $\bold{U}, \bold{V}$ be any pair of vectors of binary random variables and suppose $-C \leq \min_{\bold{U}, \bold{V}} D(\bold{U}, \bold{V})$ for some $C\in \mathbb{R}_{\geq 0}$.
$$\lim_{n\rightarrow\infty} \big(\mathbb{E}_{\bold{X}^0}\big[\max_{\eta} D(\bold{X}^1, \bold{X}^1_{\eta})\big]\big) = \lim_{n\rightarrow\infty}\big(\max_{\bold{A}, \bold{B}}D(\bold{A}, \bold{B})\big)$$
\end{theorem}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    \begin{figure}[h] \label{fig:ex1}
    \begin{center}
      \begin{tikzpicture}
\tikzset{vertex/.style = {shape = circle,fill = black,minimum size = 6pt,inner sep=0pt}}
        \tikzset{edge/.style = {-{Latex[length=2mm]}}}
      
        \node[vertex, label=left:$X_1^0$] (x10) at (0,2.5) {};
        \node[vertex, label=right:$X_1^1$] (x11) at (4,2.5) {};
        \node[vertex, label=left:$X_2^0$] (x20) at (0, 1.5) {};
        \node[vertex, label=right:$X_2^1$] (x21) at (4, 1.5) {};
        \node[vertex, label=left:$X_n^0$] (xn0) at (0, 0) {};
        \node[vertex, label=right:$X_n^1$] (xn1) at (4, 0) {};
        \draw node[fill, circle, scale = 0.3] at (2, 1.1) {};
        \draw node[fill, circle, scale = 0.3] at (2, 0.65) {};
        \draw node[fill, circle, scale = 0.3] at (2, 0.2) {};
        
        \draw[edge] (x20) to (x21);
        \draw[edge] (x20) to (x11);
        \draw[edge] (x20) to (xn1);
        \draw[edge] (x10) to (x11);
        \draw[edge] (x10) to (x21);
        \draw[edge] (x10) to (xn1);
        \draw[edge] (xn0) to (xn1);
        \draw[edge] (xn0) to (x11);
        \draw[edge] (xn0) to (x21);
      \end{tikzpicture}
    \end{center}
    \caption{Representation of the family of networks used in proposition \ref{prop:arb}}
   \end{figure}
   
%%%%%%%%%%%%%%%%%%%%%%%
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%
   
\begin{proof}
Let $\bold{A}, \bold{B}$ be the vectors of binary random variables for which $D(\bold{A}, \bold{B})$ attains its maximum value, with respect to $n$. Then $\bold{A} = \langle A_1, ..., A_n \rangle$, $\bold{B} = \langle B_1, ..., B_n \rangle$ and each variable has prior $\mathbb{P}(A_i = 1 ) = a_i$, $\mathbb{P}(B_i = 1) = b_i$.
Let $\boldsymbol{X}^0 \rightarrow \boldsymbol{X}^1$ define a dynamic Bayes network on $n$ variables. For all $1\leq j \leq n$, let $\Pa(X_j^1) = \{X_i^0: 1\leq i \leq n\}$. 
That is, all nodes in layer 0 are parents of every node in layer 1. 
The probability distributions over $\boldsymbol{X}^0$ and $\boldsymbol{X}^1$ are defined by: $\forall X_i^0\in \boldsymbol{X}^0$, $\mathbb{P}(X_i^0 = 1) = \epsilon = \frac{\log(n)}{n}$. Next, $\forall X_i^1\in\boldsymbol{X}^1$, $\mathbb{P}(X_i^1 = 1| \exists x_j^0 = 1) = a_i$ and $\mathbb{P}(X_i^1 = 1| \nexists x_j^0 = 1) = b_i$. 

%To show the desired convergence, we will prove that 
%$$\lim_{n \rightarrow \infty} \mathbb{E}[L\big(F(\boldsymbol{X}_n^t | \boldsymbol{X}_n^{t-1}\setminus\eta), F(\boldsymbol{X}_n^t | \boldsymbol{X}_n^{t-1})\big)] = L(\bold{u}, bold{v}).$$


For each $n$ we will consider the value of $D(\bold{X}^1, \bold{X}_{\eta}^1)$ under three types of events that could occur with respect to the possible outcomes, $\bold{x}^0$ of $\boldsymbol{X}^0$, the adversary's budget $k$, and the adversary's choice of which nodes to hide conditional on $\bold{x}^0$. These settings produce three unique types of adversarial play, namely
\begin{itemize}
    \item (1) $\sum_{X_j^0}x_j^0 = 0$. In this case the adversary will hide $k$ random nodes since all outcomes are 0.
    \item (2) $\sum_{X_j^0}x_j^0 = m \leq k$. In this case the adversary will hide only the $m$ nodes whose outcomes are 1.
    \item (3) $\sum_{X_j^0}x_j^0 = m > k$. In this case the adversary will hide nothing.
\end{itemize}

In events of type (1) when there is no obstruction $\bold{X}^1 = \bold{B}$. When $\eta$ is hidden,
$\bold{X}_{\eta}^1 = \bold{A}$ with probability $1-(1-\epsilon)^k$, and $\bold{X}_{\eta}^1 = \bold{B}$ with probability $(1-\epsilon)^k$.
Thus, in this setting, 
$$\mathbb{E}\big[ D(\bold{X}^1, \bold{X}_{\eta}^1 )\big] = \big(1 - (1-\epsilon)^k\big)D(\bold{B}, \bold{A}) + (1-\epsilon)^k D(\bold{B}, \bold{B})$$
Events of this type occur with probability $(1-\epsilon)^n$.

In events of type (2), without $\eta$ we have $\bold{X}^1 =  \bold{A}$. Since $m \leq k$ and all nodes with outcome 0 will be hidden, obscuring $\eta$ will cause $\bold{X}_{\eta}^1 = \bold{B}$ with probability $(1 - \epsilon)^m$, and $\bold{X}_{\eta}^1 = \bold{A}$ with probability $1 - (1-\epsilon)^m$.
Therefore, the expected value in this setting is 

$$\mathbb{E}\big[ D(\bold{X}^1, \bold{X}_{\eta}^1)\big] = \big(1 - (1-\epsilon)^m\big)D(\bold{A}, \bold{A}) + (1-\epsilon)^m D(\bold{A}, \bold{B})$$
Events of this type occur with probability $\binom{n}{m}\epsilon^m(1-\epsilon)^{n-m}$ for each $m \leq k$.

In events of type (3) there are more nodes yielding 1 in layer 0 than the adversary is capable of hiding. So $\bold{X}^1 = \bold{X}_{\eta}^1 = \bold{A}$. Events of this type occur with probability $\binom{n}{m}\epsilon^m(1-\epsilon)^{n-m}$ for each $m > h$.

For notational connivance, and without loss of generality, we will reorder the nodes in $\boldsymbol{X}_n^0$ after the observations are made by the adversary, such that for $0\leq j \leq m$, $x_j^0 = 1$.
Suppose $k = n$, similar analysis holds for any constant fraction of $n$.

$$\mathbb{E}_{\bold{X}^0}\big[\max_{\eta} D(\bold{X}^1, \bold{X}^1_{\eta})\big]$$

$$\geq D(\bold{B}, \bold{A})\big(1-(1-\epsilon)^n\big)(1-\epsilon)^n + (1-\epsilon)^{2k}D(\bold{A}, \bold{A})$$
$$+ D(\bold{A}, \bold{B})\bigg(\sum_{m=1}^n\binom{n}{m}\epsilon^m(1-\epsilon)^{n-m}(1-\epsilon)^m\bigg)$$

$$=D(\bold{A}, \bold{B})\big(1-(1-\epsilon)^n\big)(1-\epsilon)^n$$
$$+ D(\bold{A}, \bold{B})\bigg(\sum_{m=1}^n\binom{n}{m}\epsilon^m(1-\epsilon)^{n}\bigg)$$

$$=D(\bold{A}, \bold{B})\big(1-(1-\epsilon)^n\big)(1-\epsilon)^n$$
$$+ D(\bold{A}, \bold{B})(1-\epsilon)^n\bigg(\sum_{m=1}^n\binom{n}{m}\epsilon^m\bigg)$$

Using the binomial identity we can reduce the above equation to form

$$=D(\bold{A}, \bold{B})\bigg(\big(1-(1-\epsilon)^n\big)(1-\epsilon)^n + (1-\epsilon)^n \big((\epsilon+1)^n-1\big)\bigg)$$

$$ = D(\bold{A}, \bold{B}) \bigg((1-\epsilon)^n \left((\epsilon+1)^n-(1-\epsilon)^n\right)\bigg)$$

Thus it remains only to be shown that there exists a value of $\epsilon$, representing a probability, such that 
$$(1-\epsilon)^n \left((\epsilon+1)^n-(1-\epsilon)^n\right) \rightarrow 1 \text{ as } n\rightarrow \infty$$
This limit can be evaluated follows
$$\lim_{n \rightarrow \infty}(1-\epsilon)^n \left((\epsilon+1)^n-(1-\epsilon)^n\right)$$
$$ = \lim_{n \rightarrow \infty}(1-\epsilon^2)^n-\lim_{n\rightarrow\infty}(1-\epsilon)^{2n} $$
$$ = \lim_{n \rightarrow \infty}\bigg(1-\bigg(\frac{log(n)}{n}\bigg)^2\bigg)^n-\lim_{n\rightarrow\infty}\bigg(1-\bigg(\frac{log(n)}{n}\bigg)\bigg)^{2n} $$
Using a slight variation to the identity $\lim_{n\rightarrow \infty}(1+\frac{a}{n})^{c n} = e^{ac}$, we can obtain 

$$\lim_{n \rightarrow \infty}\bigg(1-\bigg(\frac{log(n)}{n}\bigg)^2\bigg)^n = 1$$
and 
$$ \lim_{n\rightarrow\infty}\bigg(1-\bigg(\frac{log(n)}{n}\bigg)\bigg)^{2n}  = 0$$

Thus giving the desired result that 
$$\lim_{n\rightarrow\infty}(1-\epsilon)^n \left((\epsilon+1)^n-(1-\epsilon)^n\right) = 1$$

%%%%%%%%%%
\iffalse
%%%%%%%%%%%%%
Using the identity that let $\lim_{n\rightarrow \infty}(1+\frac{b_n}{n})^{c n} = e^{ac}$, for any sequence $b_n$ with asymptotic behavior 
Now we have that 
$$ = \lim_{n \rightarrow \infty} \big((1- \frac{a^2}{n^2})^{n^2}\big)^{\frac{1}{n}} -\lim_{n\rightarrow\infty}(1-\frac{a}{n})^{2n}$$
$$ = \lim_{n \rightarrow \infty} e^{\frac{-1}{n}} -\lim_{n\rightarrow\infty}(1-\frac{a}{n})^{2n}$$
$$ = 1 -e^{-2a}$$



We are free to choose this value $a$ so that it maintains the invariant that $\epsilon = \frac{a}{n}$ represents a probability.
Note that for any fixed $a$, the above quantity will always be less than 1. However for values of $a$ that are functions of $n$ our analysis of the limit requires an additional step to assure convergence.
Thus, we must modify our sequence $\{\mathbb{X}_n\}_n$ to be two dimensional and encode the value of $a$.
Note that such a modification to the sequence is viable since we are taking a supremum over all possible dynamic Bayes network instances.
Let $\{\mathbb{X}_{(n, a)}\}_{(n,a)}$ denote this new sequence where $a$ constitutes a proper probability for each of its pairings with $n$. 
The supremum is now evaluated via
$$\lim_{a\rightarrow \infty} \Bigg(\lim_{n\rightarrow \infty}\mathbb{E}\bigg[L\bigg(F\big(\bold{X}_n^t|\bold{X}_n^{t-1}(\eta)\big), F\big(\bold{X}_n^t|\bold{X}_n^{t-1}\big)\bigg)\bigg]\Bigg)$$
$$=\lim_{a\rightarrow \infty} \big L(\bold{u}, \bold{v})( 1-e^{-2a}\big) = L(\bold{u}, \bold{v})$$

Therefore as $n$ and $a$ approach infinity, the observer's loss gets arbitrarily close to the maximum value of the the loss function $L$. Meaning, 
%%%%%%%%%%
\fi
%%%%%%%%%%
$$\lim_{n\rightarrow\infty} \big(\mathbb{E}_{\bold{X}^0}\big[\max_{\eta} D(\bold{X}^1, \bold{X}^1_{\eta})\big]\big) = \lim_{n\rightarrow\infty}\big(\max_{\bold{A}, \bold{B}}D(\bold{A}, \bold{B})\big)$$

\end{proof}

%\begin{corollary}
%When the loss function is any distance metric, an attacker is capable of achieving arbitrarily high utility on an infinite family of examples
%\end{corollary}

%\begin{proof}
%Follows immediately from Proposition \ref{prop:arb}
%\end{proof}


==> old.tex <==

%%%%%%%%%%%
%%%%%%%%%%%
\iffalse
%%%%%%%%%%%
%%%%%%%%%%%

\section{$L_{\infty}$ Norm}

\begin{proposition}
Consider a network consisting of states at two time steps, $\boldsymbol{X}^0$ and $\boldsymbol{X}^1$ where, $\forall X_i^1 \in \bold{X}^1, Pa(X_i^1) = \{X_i^0\}$. That is, each variable has a single dependency, namely itself at the previous time step.  
Let the number of nodes the adversary can hide be one, $h=1$. Then,
$$\sup_n\{\mathbb{E}[||\mathbb{P}(\boldsymbol{X}^t | \phi(\boldsymbol{X}^{t-1}\setminus\eta)) - \mathbb{P}(\boldsymbol{X}^t | \phi(\boldsymbol{X}^{t-1}))||_{\infty}]: n\in \mathbb{N}\} = 1$$
\\
\\
\end{proposition}

    \begin{figure}[!h] \label{fig:ex1}
    \begin{center}
      \begin{tikzpicture}
\tikzset{vertex/.style = {shape = circle,fill = black,minimum size = 6pt,inner sep=0pt}}
        \tikzset{edge/.style = {-{Latex[length=2mm]}}}
      
        \node[vertex, label=left:$X_1^0$] (x10) at (0,2.5) {};
        \node[vertex, label=right:$X_1^1$] (x11) at (4,2.5) {};
        \node[vertex, label=left:$X_2^0$] (x20) at (0, 1.5) {};
        \node[vertex, label=right:$X_2^1$] (x21) at (4, 1.5) {};
        \node[vertex, label=left:$X_n^0$] (xn0) at (0, 0) {};
        \node[vertex, label=right:$X_n^1$] (xn1) at (4, 0) {};
        \draw node[fill, circle, scale = 0.3] at (2, 1.1) {};
        \draw node[fill, circle, scale = 0.3] at (2, 0.65) {};
        \draw node[fill, circle, scale = 0.3] at (2, 0.2) {};
        
        \draw[edge] (x20) to (x21);
        \draw[edge] (x10) to (x11); 
        \draw[edge] (xn0) to (xn1);
      \end{tikzpicture}
    \end{center}
    \caption{Representation of the family of networks used in claim 2.1}
   \end{figure}

\begin{proof}
For each $X_i^0\in \bold{X}^0$ let $\mathbb{P}(X_i^0 = 1) = \frac{1}{\sqrt{n}}$, $\mathbb{P}(X_i^1=1|\phi(\{X_i^0\})=1)=1$,
and $\mathbb{P}(X_i^1=1|\phi(\{X_i^0\})=0)=0$. 
If there exists at least one $X_i^0$ with $\phi(X_i^0)= 1$, then by hiding $X_i^0$, the adversary a utility of 

$$||\mathbb{P}(\boldsymbol{X}^t | \phi(\boldsymbol{X}^{t-1}\setminus\eta)) - \mathbb{P}(\boldsymbol{X}^t | \phi(\boldsymbol{X}^{t-1}))||_{\infty} = |\frac{1}{\sqrt{n}} - 1|.$$

If there does not exist such an $X_i^0$, then hiding any $X_j^0$ yields the attacker a utility of 

$$||\mathbb{P}(\boldsymbol{X}^t | \phi(\boldsymbol{X}^{t-1}\setminus\eta)) - \mathbb{P}(\boldsymbol{X}^t | \phi(\boldsymbol{X}^{t-1}))||_{\infty} = |\frac{1}{\sqrt{n}} - 0|.$$

The probability of these events occurring is characterized by $\mathbb{P}(\exists X_i^0 = 1) = \sum_{k = 1}^n {n \choose k}(\frac{1}{\sqrt{n}})^k(1-\frac{1}{\sqrt{n}})^{n -k}$ and 
$\mathbb{P}(\nexists X_i^0 = 1) = (\frac{1}{\sqrt{n}})^n$.
Thus,

$$\mathbb{E}[||\mathbb{P}(\boldsymbol{X}^t | \phi(\boldsymbol{X}^{t-1}\setminus\eta)) - \mathbb{P}(\boldsymbol{X}^t | \phi(\boldsymbol{X}^{t-1}))||]$$
$$= \mathbb{P}(\exists X_i^0 = 1)|\frac{1}{\sqrt{n}} - 1| + \mathbb{P}(\nexists X_i^0 = 1)|\frac{1}{\sqrt{n}} - 0|$$ 
$$\leq |\frac{1}{\sqrt{n}} - 1| + \frac{1}{\sqrt{n}}|\frac{1}{\sqrt{n}} - 0| \leq 1$$

Now, for any $\epsilon > 0$, let $N = \frac{2}{\epsilon}$ and for any $n \geq N$ we get,

$$|\mathbb{E}[||\mathbb{P}(\boldsymbol{X}_n^t | \boldsymbol{X}_n^{t-1}(\eta)) - \mathbb{P}(\boldsymbol{X}_n^t | \boldsymbol{X}_n^{t-1})||] - 1|$$
$$\leq ||\frac{1}{\sqrt{n}} - 1| + \frac{1}{\sqrt{n}}|\frac{1}{\sqrt{n}} - 0| - 1| $$
$$ \leq |1 + \frac{1}{n} - 1|$$
$$ = |\frac{1}{n}| \leq |\frac{1}{2/\epsilon}| < \epsilon$$.

Thus, 
$$\sup_n~\{\mathbb{E}[||\mathbb{P}(\boldsymbol{X}_n^t | \phi(\boldsymbol{X}^{t-1}\setminus\eta)) - \mathbb{P}(\boldsymbol{X}_n^t | \phi(\boldsymbol{X}^{t-1}))||_{\infty}]:n\in\mathbb{N}\} = 1$$

\end{proof}

\section{$L_p$ Norm}

\begin{proposition} 
Let $p \in \mathbb{N}$ and let $\mathbb{X}$ be any instance of a dynamic Bayes net. Then
$$\sup_{\mathbb{X}} \frac{\mathbb{E}[||\mathbb{P}(\boldsymbol{X}^t | \boldsymbol{X}^{t-1}(\eta)) - \mathbb{P}(\boldsymbol{X}^t | \boldsymbol{X}^{t-1})||_p]}{||1||_p} = 1 $$
\\
\\
\end{proposition}

    \begin{figure}[h] \label{fig:ex1}
    \begin{center}
      \begin{tikzpicture}
\tikzset{vertex/.style = {shape = circle,fill = black,minimum size = 6pt,inner sep=0pt}}
        \tikzset{edge/.style = {-{Latex[length=2mm]}}}
      
        \node[vertex, label=left:$X_1^0$] (x10) at (0,2.5) {};
        \node[vertex, label=right:$X_1^1$] (x11) at (4,2.5) {};
        \node[vertex, label=left:$X_2^0$] (x20) at (0, 1.5) {};
        \node[vertex, label=right:$X_2^1$] (x21) at (4, 1.5) {};
        \node[vertex, label=left:$X_n^0$] (xn0) at (0, 0) {};
        \node[vertex, label=right:$X_n^1$] (xn1) at (4, 0) {};
        \draw node[fill, circle, scale = 0.3] at (2, 1.1) {};
        \draw node[fill, circle, scale = 0.3] at (2, 0.65) {};
        \draw node[fill, circle, scale = 0.3] at (2, 0.2) {};
        
        \draw[edge] (x20) to (x21);
        \draw[edge] (x20) to (x11);
        \draw[edge] (x20) to (xn1);
        \draw[edge] (x10) to (x11);
        \draw[edge] (x10) to (x21);
        \draw[edge] (x10) to (xn1);
        \draw[edge] (xn0) to (xn1);
        \draw[edge] (xn0) to (x11);
        \drwa[edge] (xn0) to (x21);
      \end{tikzpicture}
    \end{center}
    \caption{Representation of the family of networks used in claim 3.1}
   \end{figure}
   
   
   
\begin{proof}
First note that $\sup_{\mathbb{X}} \frac{\mathbb{E}[||\mathbb{P}(\boldsymbol{X}_n^t | \boldsymbol{X}_n^{t-1}(\eta)) - \mathbb{P}(\boldsymbol{X}_n^t | \boldsymbol{X}_n^{t-1})||_p]}{||1||_p}$ is bounded from above by 1. 
So, it only remains to be shown that there exists some sequence of examples $\{\mathbb{X}_n\}_n$ such that,
$$\lim_{n \rightarrow \infty} \frac{\mathbb{E}[||\mathbb{P}(\boldsymbol{X}_n^t | \boldsymbol{X}_n^{t-1}(\eta)) - \mathbb{P}(\boldsymbol{X}_n^t | \boldsymbol{X}_n^{t-1})||_p]}{||1||_p} = 1 $$
Such a sequence will be defined as follows. 
Let $\mathbb{X}_n = \boldsymbol{X}_n^0 \rightarrow \boldsymbol{X}_n^1$ where both $\boldsymbol{X}_n^i = \{X_1^i, ..., X_n^i\}$ for $i\in \{0, 1\}$. For all $1\leq j \leq n$, let $\Pa(X_j^1) = \{X_k^0: 1\leq k \leq n\}$. 
That is, all nodes in layer 0 are parents of every node in layer 1. 
The probability distributions over $\boldsymbol{X}_n^0$ and $\boldsymbol{X}_n^1$ are defined by: $\forall X_i^0\in \boldsymbol{X}_n^0$, $\mathbb{P}(X_i^0 = 1) = q$ a value that we will assing later, $\forall X_i^1\in\boldsymbol{X}_n^1$, $\mathbb{P}(X_i^1 = 1| \exists X_j^0 = 1) = 1$ and $\mathbb{P}(X_i^1 = 1| \nexists X_j^0 = 1) = 0$. 

To show the desired convergence, we will prove that 
$$\lim_{n \rightarrow \infty} \mathbb{E}[\mathbb{P}(\boldsymbol{X}_n^t | \boldsymbol{X}_n^{t-1}(\eta)) - \mathbb{P}(\boldsymbol{X}_n^t | \boldsymbol{X}_n^{t-1})] = <1, 1, ..., 1>.$$
To accomplish this, we will show that the element-wise absolute difference converges to 1 for each pair of elements in the above two vectors. That is,
$$\forall X_i^1\in\boldsymbol{X}_n^1,~\lim_{n\rightarrow\infty}\mathbb{E}[|\mathbb{P}(X_i^1|\phi(Pa(X_i^1) \setminus \eta) - \mathbb{P}(X_i^1|Pa(X_i^1)|] = 1$$
For each $n$ we will consider the above value under three types of events that could occur based off the outcomes of $\boldsymbol{X}_n^0$, the adversaries budges $h$, and the adversaries choice of which nodes to hide.
\begin{itemize}
    \item (1) $\sum_{X_j^0}X_j^0 = 0$. In this case the adversary will hide $h$ random nodes since all outcomes are 0.
    \item (2) $\sum_{X_j^0}X_j^0 = m \leq h$. In this case the adversary will hide all $m$ nodes whose outcome was 1.
    \item (3) $\sum_{X_j^0}X_j^0 = m > h$. In this case the adversary hides nothing.
\end{itemize}

In events of type (1) the true value of all nodes in $\boldsymbol{X}_n^1$ is $X_j^1 = 0$, since $h$ nodes are hidden, the observer will use the prior belief to predict the probability that at least one of those nodes is 1. 
Events of this type occur with probability $(1-q)^n$.
In events of type (2) the true value of all nodes in $\boldsymbol{X}_n^1$ is $X_j^1 = 1$. Since $m$, the number of outcomes in layer 0 that are one, is less or equal to $h$ and all such nodes are hidden, the observer will again use its prior belief to predict the probability that at least one of the hidden nodes is 1.
These events occur with probability $\binom{n}{m}q^m(1-q)^{n-m}$ with $m \leq h$
In events of type (3) there are more nodes yielding one in layer 0 than the adversary is capable of hiding. Since the transition function of all nodes from layer 0 to 1 is defined deterministicly on the 
outcome of at least one node in layer 0 being 1, the observer will make perfect predictions independent of the adversaries actions. This type of event occurs with probability $\binom{n}{m}q^m(1-q)^{n-m}$ with $m > h$.
For notational connivance, and without loss of generality, we will reorder the nodes in $\boldsymbol{X}_n^0$ after the observations are made by the adversary, such that for $0\leq j \leq m$, $X_j = 1$.
Suppose $h = n$, then we have,


$$\mathbb{E}[|\mathbb{P}(X_i^1|\phi(Pa(X_i^1)\setminus \eta) - \mathbb{P}(X_i^1|\phi(Pa(X_i^1))|] $$
$$ = \bigg(\sum_{m=1}^n \mathbb{P}(\sum_{j\leq n}X_j^0 = m)\bigg|\mathbb{P}(\sum_{k \leq m}X_j^0 \geq 1) - 1\bigg|\bigg)$$
$$+ \mathbb{P}(\sum_{j\leq n} X_j^0 = 0)\bigg|1 - 0\bigg|$$
$$=\bigg(\sum_{m = 1}^n\binom{n}{m}q^m(1-q)^{n-m}\bigg|1-(1-q)^m - 1\bigg| \bigg)$$
$$+ (1-q)^n\bigg|1-(1-q)^n\bigg|$$
$$=\bigg(\sum_{m = 1}^n\binom{n}{m}q^m(1-q)^{n-m}(1-q)^m\bigg) + (1-q)^n(1-(1-q)^n)$$
$$=(1-q)^n\bigg(\sum_{m = 1}^n\binom{n}{m}q^m\bigg) + (1-q)^n(1-(1-q)^n)$$

Using the binomial identity we can reduce the above equation to form

$$=(1-q)^n\big((1+q)^n-1\big) + (1-q)^n\big(1-(1-q)^n\big)$$
$$=(1-q)^n \big((q+1)^n-(1-q)^n\big)$$
Thus it remains only to be shown that there exists a value of $q$ such that 
$$(1-q)^n \big((q+1)^n-(1-q)^n\big) \rightarrow 1 \text{ as } n\rightarrow \infty$$
This limit can be evaluated follows
$$\lim_{n \rightarrow \infty}(1-q)^n \big((q+1)^n-(1-q)^n\big)$$
$$= \lim_{n \rightarrow \infty}(1-q)^n \big(\lim_{n \rightarrow \infty}(1+q)^n-\lim_{n \rightarrow \infty}(1-q)^n\big)$$

Now let $q = \frac{a}{n}$ for some arbitrary $a \in \mathbb{Z}$ which will be specified later.
Then, each of these limits is in the form $\lim_{n \rightarrow \infty}(1+\frac{b}{n})^n$ for $b = -+ a$.
Suppose the limit of such a sequence exists, say $l_b = \lim_{n \rightarrow \infty}(1+\frac{b}{n})^n$.
Then we have, 
$$\ln{l_b} = \lim_{n \rightarrow \infty}\frac{\ln{(1+\frac{b}{n})}}{1/n}$$
Not that both the numerator and denominator of this limit are differentiable for $n > 0$ and tend towards 0 as $n$ tends towards $\infty$.
Therefore, L'Hopital's rules gives that
$$ \lim_{n \rightarrow \infty}\frac{\ln{(1+\frac{b}{n})}}{1/n} = \lim_{n \rightarrow \infty}\frac{\frac{1}{(1+\frac{b}{n})(-\frac{b}{n^2})}}{-1/n^2}$$
$$ =\lim_{n\rightarrow\infty}\frac{b}{1+\frac{b}{n}} = \frac{b}{1+\lim_{n\rightarrow\infty}(\frac{b}{n})} = \frac{b}{1 + 0} = b$$
Hence, $l_b = e^b$, and 
$$= \lim_{n \rightarrow \infty}(1-\frac{a}{n})^n \big(\lim_{n \rightarrow \infty}(1+\frac{a}{n})^n-\lim_{n \rightarrow \infty}(1-\frac{a}{n})^n\big)$$
$$=e^{-a}\big(e^a - e^{-a}\big) = 1-e^{-2a}$$.

Now we have that 
$$\lim_{n\rightarrow \infty}\mathbb{E}[|\mathbb{P}(\phi(X_i^1|Pa(X_i^1)\setminus \eta) - \mathbb{P}(X_i^1|Pa(X_i^1)|] = 1-e^{-2a}$$

We are free to choose this value $a$ so that it maintains the invariant that $q = \frac{a}{n}$ represents a probability.
Not that for any fixed $a$, the above quantity will always be less than 1. And for values of $a$ that are functions of $n$ our analysis of the limit does not hold.
Thus we must modify our sequence $\{\mathbb{X}_n\}_n$ to be two dimensional and encode the value of $a$.
Note that such a modification to the sequence is viable since we are taking a supremum over all possible dynamic Bayes net instances.
Let $\{\mathbb{X}_{(n, a)}\}_{(n,a)}$ denote this new sequence where $a$ constitutes a proper probability for each of its pairings with $n$. 
The supremum is now evaluated via
$$\lim_{a\rightarrow \infty} \Bigg(\lim_{n\rightarrow \infty}\mathbb{E}[|\mathbb{P}(\phi(X_i^1|Pa(X_i^1)\setminus \eta) - \mathbb{P}(X_i^1|Pa(X_i^1)|]\Bigg)$$
$$=\lim_{a\rightarrow \infty} \big( 1-e^{-2a}\big) = 1$$
Thus, as $a\rightarrow \infty$ and $n\rightarrow \infty$ the element-wise absolute difference between the observer's predictions when the adversary hides nodes, and when there is no adversary, approaches 1.
Since each each $l_p$ norm being investigated is for a fixed $p$, we have that the value of the supremum is independent of $p$.
Thus, 
$$\sup_{\mathbb{X}} \frac{\mathbb{E}[||\mathbb{P}(\boldsymbol{X}_n^t | \boldsymbol{X}_n^{t-1}(\eta)) - \mathbb{P}(\boldsymbol{X}_n^t | \boldsymbol{X}_n^{t-1})||_p]}{||1||_p} = 1 $$

\end{proof}


%%%%%%%%%%%%
%%%%%%%%%%%
\fi
%%%%%%%%%%
%%%%%%%%%%

==> rationallimit.tex <==
\subsection{Rational Observer}

Similar to Proposition \ref{prop:arb} we demonstrate the maximum impact an attack can have on a ration observer. However, we cannot make such a claim over all positive symmetric loss functions. To see this, one could imagine a loss function over the true value of $\bold{X}_n^t$, $\bold{u}$ and the observer's guess of the state of $\bold{X}_n^t$, $\bold{v}$, defined by $L(\bold{u}, \bold{v}) = 0$ if $\exists u_i = v_i$ and $L(\bold{u}, \bold{v}) = 1$ otherwise. In this setting, over any dynamic Bayes network we know that for each $X_i^t\in\bold{X}_n^t$ either $\mathbb{P}(X_i^t = 1) \geq \frac{1}{2}$ or $\mathbb{P}(X_i^1 = 0 ) \geq \frac{1}{2}$. Thus, for any outcome $\phi$, the observer could simply guess $\text{argmax}\{ \mathbb{P}(X_i^t = a)\}, a\in \{0, 1\}$ for each $1\leq i\leq n$ and would achieve a loss of 0 with probability at least $1 - \frac{1}{2^n}$. Hence the observer can be arbitrarily correct over this loss function for $n$ sufficiently large. 

Although a statement cannot be made about loss functions in general, we will examine one specific loss function, the expected Hamming distance. The Hamming distance is defined as $H(\bold{v}, \bold{u}) = \sum_{i = 1}^n \mathbb{I}(u_i = v_i)$. Intuitively this metric can be thought of as the number of nodes in $\bold{X}_n^t$ for which the observer predicts the wrong outcome. As this loss function is a representation of the observers incorrect predictions, it is a natural metric to consider and will be our primary focus throughout the rest of the paper, although many of the results provided either hold for, or are easily extended to, other common loss functions. 


\begin{claim}
There exists an infinite family of dynamic Bayes networks over which a rational observer can be forced into an expected loss of $\frac{n}{2}$, half of optimal, when $L\bigg(F\big(\bold{X}_n^t|\bold{X}_n^{t-1}(\eta)\big), F(\bold{X}_n^t|\bold{X}_n^{t-1}(\emptyset)\big)\bigg) = H\bigg(F\big(\bold{X}_n^t|\bold{X}_n^{t-1}(\eta)\big), F(\bold{X}_n^t|\bold{X}_n^{t-1}(\emptyset)\big)\bigg)$
\end{claim}

\begin{proof}
Consider a dynamic Bayes network of the following from. 
For each $X_i^{t -1} \in \bold{X}_n^{t-1}$, let $\mathbb{P}{(X_i^{t-1} = 1) = \frac{1}{2}}$, and for each $X_i^t\in\bold{X}_n^t$ let $\Pa(X_i)^t = \{X_i^{t-1}, X_{i+1}^{t-1}\}$, with the understanding that if $i = n$, then the index $i+1 = 1$. Lastly, let $\mathbb{P}{(X_i^t = \phi(X_i^{t-1}) \text{XOR} \phi(X_{i+1}^{t-1}) |\phi(\Pa(X_i^t)) = 1}$. Suppose that the attacker's budget is $k = \frac{n}{2}$. Then, the optimal strategy for the attacker is to randomly choose one node from each $\Pa(X_i^t)$ to hide independent of $\phi$. Under this scheme, the observer gains no information as to the outcomes based on the mask $\eta$, in the sense that the observer cannot deduce what outcomes the attacker was shown, since the attacker makes their decision independent of the outcome map. As a result the observer has only the priors and the transition probability to make a prediction about the outcomes of $\bold{X}^t$. Since the observer sees only a single outcome of each parent set $\Pa(X_i^t)$, and the the value of $X_i^t$ is precisely the XOR of its parents, the observer best strategy is to guess that the outcome of each $X_i^t$ is 1 with probability $\frac{1}{2}$ and to guess 0 with probability $\frac{1}{2}$. In this case, the expected hamming distance on each node is given by $H(\frac{1}{2}, \phi(X_i^t)\text{XOR} \phi(X_{i+t}^1) = \frac{1}{2}$. Thus the total loss of the observer, i.e. the sum over the expected hamming distance on each node, is $\frac{n}{2}$. 
\end{proof}


